Using Fitts' Law to Benchmark Assisted Human-Robot Performance

Shared control systems aim to combine human and robot abilities to improve task performance. However, achieving optimal performance requires that the robot's level of assistance adjusts the operator's cognitive workload in response to the task difficulty. Understanding and dynamically adjusting this balance is crucial to maximizing efficiency and user satisfaction. In this paper, we propose a novel benchmarking method for shared control systems based on Fitts' Law to formally parameterize the difficulty level of a target-reaching task. With this we systematically quantify and model the effect of task difficulty (i.e. size and distance of target) and robot autonomy on task performance and operators' cognitive load and trust levels. Our empirical results (N=24) not only show that both task difficulty and robot autonomy influence task performance, but also that the performance can be modelled using these parameters, which may allow for the generalization of this relationship across more diverse setups. We also found that the users' perceived cognitive load and trust were influenced by these factors. Given the challenges in directly measuring cognitive load in real-time, our adapted Fitts' model presents a potential alternative approach to estimate cognitive load through determining the difficulty level of the task, with the assumption that greater task difficulty results in higher cognitive load levels. We hope that these insights and our proposed framework inspire future works to further investigate the generalizability of the method, ultimately enabling the benchmarking and systematic assessment of shared control quality and user impact, which will aid in the development of more effective and adaptable systems.

==> intro_ideas.tex <==
Train of motivation
\begin{itemize}
    \item In HRI, shared control aims to combine the respective strengths of the human and robot to achieve better task performance overall. While humans are good at high-level planning and goal-setting, robots are good at efficiently executing precise movements (here we assume and use a high-performing robot).
    \item Previous work in HRI have shown that varying the level of robot autonomy in shared control can impact the human operator's internal state including cognitive load and trust \tocite{} levels, thus highlighting the importance of considering these human factors when designing effective and adaptive shared control systems.
    \item However, it is currently unclear how the relationship between robot autonomy and the human's internal state varies across tasks with different levels of difficulty.
    \item Furthermore, there is no existing understanding of how varying levels of robot autonomy affects the effective task difficulty as perceived by the operator \tocheck{}, and the latter's relationship with cognitive load and trust.
    \item Having such understandings would be beneficial to the design of adaptive robots which adjust their level of autonomy according to both the task difficulty and the user's state. 
    \item In addition, understanding the relationship between these variables also allows us to dynamically vary the effective difficulty level of the given task through adjusting the autonomy level of the robot in real-time according to the user's internal state. This would better inform the design of rehabilitation robots which can facilitate more efficient and effective motor learning.
    \item Since cognitive load is hard to capture in real-time, can we use the real-time ``effective" task difficulty as an approximation of the user's workload, if it correlates well with the cognitive load measures. [HAS OTHERS NOT DONE THIS YET?]
\end{itemize}

The main research questions of this study are:
\begin{enumerate}
    \item How does task difficulty and robot autonomy affect the task completion time?
    \begin{itemize}
        \item How does difficulty affect movement time based on robot autonomy?
        \item How does autonomy affect/determine the effective difficulty of the task?
        \item How does the shared control parameter relate to the effective blending parameter as measured through the robot and human movement times?
    \end{itemize}
    \item How does task difficulty and robot autonomy affect cognitive load?
    \begin{itemize}
        \item How does the nominal task difficulty, effective difficulty, and measured cognitive load correlate?
    \end{itemize}
    \item How does task difficulty and robot autonomy affect trust?
    \item How does the human and robot take different roles in distality control?
    \begin{itemize}
        \item Human for rough movement?
        \item Robot for fine adjustments?
    \end{itemize}
\end{enumerate}

==> old_intro.tex <==
In Human-Robot Interaction (HRI), shared control aims to combine the respective strengths of the human and robot to achieve better task performance and reduce user workload. However, when evaluating shared control systems that optimize for performance and user perception, existing HRI studies mostly employ tasks such as reaching \cite{lin2020shared, jain2019probabilistic} and pick-and-place motions \cite{young2019formalized, munguia2023affordance} which are loosely defined, leading to a lack of formal quantification of task difficulty \cite{leichtmann2022crisis}. Here, the level of difficulty is an important aspect of a task as it has been shown to affect the user's performance and cognitive load during shared control \cite{luo2021workload, melnicuk2021effect, bequette2020physical}. Therefore, while these experiments serve to validate improvements in performance and/or user perception through using shared control, the lack of a formal definition of task difficulty impacts the replicability and real-world transferability of these results \cite{leichtmann2022crisis}. This therefore motivates the development of a benchmarking method which both allows for systematic evaluation of the quality of shared control designs and enables fair and informative comparisons against alternative approaches.

Fitts' Law \cite{fitts1954information} is a benchmarking framework used extensively in Human-Computer Interaction (HCI) research to evaluate control interface designs \cite{argelaguet2013survey, drewes2010only, so2000effects}. It provides a formal definition of an \textit{index of difficulty} for reaching motions and models the relationship between difficulty and human performance (See Section \ref{related:fitts_law}). However, to successfully apply Fitts' Law as a benchmarking method to evaluate shared control systems in HRI, we need to understand how different levels of robot autonomy may impact the difficulty-performance relationship predicted by Fitts' Law. Such an understanding could also provide insights into how we may use Fitts' Law as a predictor of task performance to inform real-time adaptation of the level of robot assistance during shared control.
% Given the challenges of objectively quantifying and reliably measuring humans' internal state in real-time \cite{marchand2021measuring},

Motivated by the above aspects, the overarching research question of this study is: \textit{How does task difficulty and robot autonomy affect the user's performance and cognitive load?}
To better understand this relationship, we conducted a teleoperation study using a target reaching task with a definition of difficulty based on Fitts' Law (See Section \ref{method:task}), and a shared-control scheme which allowed continuous variation of robot autonomy \footnote{The code and data, along with a demo video of the experiment, are available on the project website: \href{https://sites.google.com/view/autonomyfitts/home}{https://sites.google.com/view/autonomyfitts/home}.}. Through both objective and subjective measures of task performance and cognitive workload, and the use of Fitts' Law which allowed a more formal and generalizable evaluation of the effects of robot autonomy on our measures under systematic variation of task difficulty, we aimed to uncover the impact of task difficulty and level of robot assistance on these variables.

To summarize, this paper aims to contribute in the following aspects:
\begin{enumerate}
    \item We investigate the effects of task difficulty and autonomy on the users' performance and cognitive load in a shared control task.
    \item We propose an adapted Fitts' Law as a benchmarking method for evaluating shared control systems, which allows to capture the interaction between task difficulty and robot assistance on user performance.
\end{enumerate}

==> rebuttal_points.tex <==
% THINGS TO DO

1. [Parallels to similar HCI studies] Given that existing HCI studies evaluating 3D user-interface design such as [1] have employed the same task of reaching towards a ring of targets in a fixed order, we agree with the AC and R3 that it is worth discussing the potential resonance and transfer of research findings across these adjacent fields. 
[DONE]
Why may findings using Fitts' Law in HCI be useful towards HRI and HRC research?
- In AR-assisted teleoperation, it might help to design a interface that is both intuitive for the user and also efficient for task completion.

2. [Benchmark as starting point for future work] Highlight this point - Thus, we believe that our proposed framework will inspire researchers to further develop and adapt the framework to bring it closer to more realistic and challenging teleoperation tasks.
[DONE]

3. [Generalizability of our chosen task, need further validation] We will therefore clarify this motivation (that reaching motions are a critical component common to most complex real-world tasks e.g. surgical, industrial) and tone down the generalizability of our chosen task, and emphasize the need for further investigation with more complex, realistic teleoperation tasks to achieve a more robust human-robot performance model.
[DONE]

4. [Cognitive load estimation] Tone down our claims around real-time cognitive load estimation using the proposed model require further validation, and and outline possible ways for future studies to extend the performance model for online cognitive load estimation.
[DONE]

5. [Discussion on trust] we will reduce the discussion on trust to avoid overstating its significance given it was not part of the study’s main objectives, but will discuss the merit of investigating trust with a noisy autonomous robot controller or with limited feedback to the user as the results are likely to be different [3]. 
[DONE]

6. [Eye-tracking information] While we did record pupil diameter using eye-tracking, the data was unreliable due to device mis-calibration, and was therefore discarded from the results and analysis. We thank the reviewers for noticing, and will make this clear in the Methods and Results sections of the revised manuscript.
[DONE]

7. [Experiment and study description / details] we will improve the clarity in the experiment and task descriptions, including that users were controlling a real robot arm instead of in simulation, that no haptic feedback was used, and other task aspects such as the controller mapping law, the criteria for successful target selection, and the simultaneous movement of the user and the robot.
[DONE]

8. [Separate recording of human/robot, results from analysis of human-only movement] Our initial analysis had shown that users were more in-sync with the robot and moved faster under higher autonomy. As the reviewers suggested, we will include these numerical results and statistical analysis to strengthen our claim.
[DONE]

9. [Terminology] we will ensure consistent terminology throughout the manuscript, including replacing "manipulation" with "reaching" which is the correct description of our chosen task. (and also assistance and autonomy)
[DONE]

10. [Related works] Relevant references, including a review of shared control methods for different robot tasks,
[DONE]

11. [Writing] improvements in punctuation and style for better readability
[DONE]

==> unused.tex <==
% \begin{itemize}
%     \item How does difficulty affect movement time based on robot autonomy?
%     \item How does autonomy affect/determine the effective difficulty of the task?
%     \item How does the shared control parameter relate to the effective blending parameter as measured through the robot and human movement times?
% \end{itemize}


% \begin{itemize}
%     \item How does the nominal task difficulty, effective difficulty, and measured cognitive load correlate?
% \end{itemize}
% \textbf{RQ3} How does task difficulty and robot autonomy affect trust?
% \textbf{RQ4} How does the human and robot take different roles in distality control?
% \begin{itemize}
%     \item Human for rough movement?
%     \item Robot for fine adjustments?
% \end{itemize}


% In addition, understanding the relationship between these variables also allows us to dynamically vary the effective difficulty level of the given task through adjusting the autonomy level of the robot in real-time according to the user's internal state. This would better inform the design of rehabilitation robots which can facilitate more efficient and effective motor learning. [This is called assist-as-needed rehab robots, previous research has shown that goal-directed movement tasks results in optimal motor learning results.]

% \begin{itemize}
%     \item In HRI, shared control aims to combine the respective strengths of the human and robot to achieve better task performance overall. While humans are good at high-level planning and goal-setting, robots are good at efficiently executing precise movements (here we assume and use a high-performing robot).
%     \item Previous work in HRI have shown that varying the level of robot autonomy in shared control can impact the human operator's internal state including both cognitive load and trust \tocite{} levels, thus highlighting the importance of considering these human factors when designing effective and adaptive shared control systems.
%     \item However, it is currently unclear how the relationship between robot autonomy and the human's internal state varies across tasks with different levels of difficulty.
%     \item Furthermore, there is no existing understanding of how varying levels of robot autonomy affects the effective task difficulty as perceived by the operator \tocheck{}, and the latter's relationship with cognitive load and trust.
%     \item Having such understandings would be beneficial to the design of adaptive robots which adjust their level of autonomy according to both the task difficulty and the user's state. 
%     \item In addition, understanding the relationship between these variables also allows us to dynamically vary the effective difficulty level of the given task through adjusting the autonomy level of the robot in real-time according to the user's internal state. This would better inform the design of rehabilitation robots which can facilitate more efficient and effective motor learning. [This is called assist-as-needed rehab robots, previous research has shown that goal-directed movement tasks results in optimal motor learning results.]
%     \item Since cognitive load is hard to capture in real-time, can we use the real-time ``effective" task difficulty as an approximation of the user's workload, if it correlates well with the cognitive load measures. [HAS OTHERS NOT DONE THIS YET?]
% \end{itemize}



% In contrast to the above results, no clear effects on the \textit{pupil diameter index} was found from both \textit{autonomy} (\(F(2,46)=.073, p=.929, \eta^2=.00058\)) and \textit{difficulty} (\(F(3,69)=1.743, p=.166, \eta^2=.013\)), and no interaction effect was observed (\(F(6,138)=1.363, p=.234, \eta^2=.024\)) on the measure. Therefore while the subjective NASA-TLX evaluation indicated that users in general perceived lower cognitive load when the robot had higher autonomy, the objective physiological measure did not show the same effect.



% Similarly, the \textit{autonomy level} was also observed to affect the \textit{single-scale trust} measure (\(F(1, 22)=33.169, p<.001, \eta^2=.234\)). Here, Pearson correlation analysis between averaged \textit{MDMT} and data from the \textit{single-scale trust} question found these two measures to be strongly positively correlated (\(r(46) = .873\), \(p < .001\)). Overall, these results indicate that users had higher trust under the \textit{high autonomy} condition, despite having lower control authority in this condition. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Adaptation of Fitts' Law Based on Autonomy} \label{results:adapted_fitts}
Given the interaction effect between \textit{difficulty} and \textit{autonomy} on the \textit{movement time} (see Section \ref{results:movement_time}), it is worth examining how exactly the Fitts relationship - which holds as expected under zero robot autonomy - needs to adapt in order to account for the influence from the continuous variation of robot autonomy.

We applied a Linear Mixed Model (LMM) to study the effects of \textit{autonomy} and \textit{difficulty} and their interaction on \textit{movement time}. Results indicated a clear slope of \textit{difficulty} on the measure (\(\beta=0.535, SE=0.026, t(100.441)=20.256, p<.001\)). While the slope of \textit{autonomy} was not statistically significant (\(\beta=-0.085, SE=0.183, t(257.01)=-0.463, p=.644\)), a clear interaction effect of \textit{difficulty} and \textit{autonomy} was observed (\(\beta=-0.177, SE=0.048, t(249.292)=-3.659, p<.001\)). This is consistent with the ANOVA results presented in Section \ref{results:movement_time}, that while there is an increase in \textit{movement time} across increasing \textit{difficulty} levels as predicted by the original Fitts' Law, the slope of this positive trend decreases under higher \textit{autonomy} levels of the robot (see Figure \todo{}).
% The model included the two independent variables and their interaction as fixed effects while accounting for individual random effects across subjects.

Based on the results from the Linear Model, an adapted Fitts equation with both \textit{index of difficulty} (ID) and \textit{robot autonomy} (\(\gamma\)) and their interaction can be derived:
\begin{equation}
\begin{aligned}
    \mathrm{MT} &= c + m_1 \mathrm{ID} + m_2 \gamma + m_3 (\gamma \cdot \mathrm{ID}) \\
    &= (c + m_2 \gamma) + (m_1 + m_3 \gamma) \cdot \mathrm{ID}  \\
    &= \tilde{a} + \tilde{b} \cdot \mathrm{ID} \\
\end{aligned}
\label{eqn:auto_fitts}
\end{equation}
where
\begin{align}
    \tilde{a} = c + m_2 \gamma &= -0.28 - 0.08 \gamma \\
    \tilde{b} = m_1 + m_3 \gamma &= 0.535 - 0.177 \gamma
\end{align}
are the coefficients obtained from our experiment. Here, both the adapted intercept \(\tilde{a}\) and the adapted slope \(\tilde{b}\) decrease across increasing autonomy levels which suggests that the robot assistance improves user task performance.



% A Linear Mixed Model indicated a clear slope of \textit{difficulty} on the measure (\(\beta=0.535, SE=0.026, t(100.441)=20.256, p<.001\)). While the slope of \textit{autonomy} was not statistically significant (\(\beta=-0.085, SE=0.183, t(257.01)=-0.463, p=.644\)), a clear interaction effect of \textit{difficulty} and \textit{autonomy} was observed (\(\beta=-0.177, SE=0.048, t(249.292)=-3.659, p<.001\)). This is consistent with the ANOVA results presented in Section \ref{results:movement_time}, that while there is an increase in \textit{movement time} across increasing \textit{difficulty} levels as predicted by the original Fitts' Law, the slope of this positive trend decreases under higher \textit{autonomy} levels of the robot (see Figure \todo{}).
% The model included the two independent variables and their interaction as fixed effects while accounting for individual random effects across subjects.




% This provides a more direct path towards designing adaptive robots which vary their level of autonomy based on both task difficulty and the user's workload.

% Furthermore, our results indicated that larger movement amplitudes yielded faster human movements, and smaller targets in general resulted in slower movements from the user. This result is consistent with the expected effects of movement amplitude and target width on the user's movement in the classic Fitts' reaching paradigm.

% We further investigated the recorded trajectories of the human to better understand the effects of robot assistance on human movement in our shared control teleoperation setting.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Human Movement Average Velocity}
% We further investigated how the average velocities of the recorded human movements varied across different task difficulty and robot autonomy levels. ANOVA showed clear effects of both \textit{difficulty} (\(F(3,69)=289.900, p<.001, \eta^2=.656\)) and \textit{autonomy} (\(F(2,46)=65.252, p<.001, \eta^2=.183\)) on the mean velocity of the human movements, and an interaction effect (\(F(3.66,84.14)=17.082, p<.001, \eta^2=.125\)) on the measure. Post-hoc comparisons indicated differences in nearly all pairs of \textit{autonomy} levels for each \textit{difficulty} level (\(p<.05\)) (see Figure \todo{}). Further post-hoc results showed differences for all pairs of \textit{difficulty} levels across all autonomy levels (\(p<.05\)), except for the \{low, med1\} \textit{difficulty} level pair under both \textit{med} and \textit{high} \textit{autonomy} levels. The plot (Figure \todo{}) suggests that higher robot assistance resulted in the user moving at higher velocities. Interestingly, it is worth noting here that despite having higher difficulty levels, rings 3 and 4 - which require larger movement amplitudes than rings 1 and 2 - yielded higher human movement velocities. Furthermore, comparing rings with different target widths (e.g. rings 1 \& 2, ring 3 \& 4), there exists a trend where smaller targets resulted in slower movements from the users.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Human Movement After Robot Finishes}
% As the robot was designed to complete the motion faster than the average user in the shared control setup, we further examined how Fitts' Law applies to the human movement after when the robot has finished its component of the motion and stopped moving. We first analyzed how the user's remaining distance to target (when the robot finishes) varies across different \textit{difficulty} and \textit{autonomy} levels. ANOVA indicated clear effects for both \textit{difficulty} (\(F(1.75,40.15)=4.055, p=.03, \eta^2=.019\)) and \textit{autonomy} (\(F(2,46)=47.005, p<.001, \eta^2=.189\)), and a clear interaction effect (\(F(6,138)=2.253, p=.042, \eta^2=.015\)). Here, it is worth highlighting that the post-hoc comparisons indicated that there was nearly no differences observed for all the \textit{difficulty} level pairs across all \textit{autonomy} levels. This means that for each level of robot assistance, the users always arrived at the same distance from the target when the robot had finished, regardless of which target ring was used.

% We then computed the Fitts \textit{index of difficulty} for the remaining sections of the human movement, using Equation \eqref{eqn:fitts_og}, and the user's remaining distance to target and the target width as the amplitude and width respectively. We applied a LMM to investigate whether a similar linear Fitts relationship between \textit{difficulty} and \textit{movement time} holds and how it varies under different \textit{autonomy} levels.

% Results indicated a clear slope of \textit{difficulty} on \textit{movement time} (\(\beta=0.403, SE=0.029, t(58.034)=13.793, p<.001\)). While the slope of \textit{autonomy} was not statistically significant (\(\beta=-0.112, SE=0.116, t(173.156)=-0.959, p=.339\)), a clear interaction effect was observed (\(\beta=-0.188, SE=0.049, t(214.585)=-3.845, p<.001\)) (Figure \todo{}). This suggests that Fitts' Law holds for the human-only movement sections, and similar to the findings presented in Section \ref{results:adapted_fitts}, this relationship adapts to the level of robot autonomy.


% we encourage future works to explore using the model as a predictor of performance to inform real-time adaptation of the level of robot autonomy based on task difficulty during shared control. 

% we aim for the proposed equation to be used as a predictor of performance to inform real-time adaptation of the level of robot autonomy based on task difficulty during shared control. 

% We propose the above equation as an adapted Fitts' performance model to more accurately capture the interaction between task difficulty and robot autonomy on movement time.

% Our results indicate that robot autonomy impacts the performance prediction model of the original Fitts' Law, thereby motivating the development of an adapted performance model which more accurately captures the interaction effects between task difficulty and robot autonomy. 

% Fitts' style interpretation of the coefficients

% These coefficients imply that robot assistance alleviates the increasing trend in movement time across increasing Fitts' ID as predicted by the traditional Fitts' Law. An alternative perspective is that higher Fitts' ID negatively impacts the gain in task performance with more robot autonomy.

% We aim for the proposed adapted Fitts' Law to contribute towards enhancing the design of adaptive shared control systems in two aspects. 

% First, the lack of formal difficulty quantification in existing HRI tasks hinders the replicability of the results and makes comparisons with different studies less informative. 

% Finally, we highlight that the coefficients of the adapted model presented above may be limited to the experimental setup of this study and thus requires further validation in alternative scenarios of human-robot shared control to enhance the generalization of our findings.

% Here, both the adapted intercept \(a(\gamma)\) and the adapted slope \(b(\gamma)\) are functions of autonomy and decrease across increasing autonomy levels which is consistent with the finding that robot assistance improves user task performance. 



%%%%% Michaels
%Human-Robot Collaboration (HRC) aims to combine the respective strengths of the human and robot to achieve better task performance and reduce user workload. However, existing evaluations of HRC systems mostly employ simple tasks such as reaching \cite{lin2020shared, jain2019probabilistic} and pick-and-place motions \cite{young2019formalized, munguia2023affordance} to validate targeted aspects of the system, and are not reflective of the tasks and actions that practical use may consider. Furthermore, these tasks are often loosely defined and lack formal quantification of task difficulty, thereby impacting the replicability and generalizability of these results \cite{leichtmann2022crisis}. Here, the level of difficulty of a task has been shown to affect the user's performance and cognitive load during HRC \cite{luo2021workload, melnicuk2021effect, bequette2020physical}, and thus should be considered when designing these systems. 

% provides a formal definition of an \textit{index of difficulty} for reaching motions and models the relationship between difficulty and human performance (See Section \ref{related:fitts_law}).
% motivates the development of a benchmarking method which both allows for systematic evaluation of the quality of shared control designs and enables fair and informative comparisons against alternative approaches.
% Fitts' Law \cite{fitts1954information} is a benchmarking framework used extensively in Human-Computer Interaction (HCI) research to evaluate control interface designs \cite{argelaguet2013survey, drewes2010only, so2000effects}. It provides a formal definition of an \textit{index of difficulty} for reaching motions and models the relationship between difficulty and human performance (See Section \ref{related:fitts_law}).
